Medusa: Universal Feature Learning via Attentional Multitasking

Recent approaches to multi-task learning (MTL) have focused on modelling connections between tasks at the decoder level. This leads to a tight coupling between tasks, which need retraining if a new task is inserted or removed. We argue that MTL is a stepping stone towards universal feature learning (UFL), which is the ability to learn generic features that can be applied to new tasks without retraining. We propose Medusa to realize this goal, designing task heads with dual attention mechanisms. The shared feature attention masks relevant backbone features for each task, allowing it to learn a generic representation. Meanwhile, a novel Multi-Scale Attention head allows the network to better combine per-task features from different scales when making the final prediction. We show the effectiveness of Medusa in UFL (+13.18% improvement), while maintaining MTL performance and being 25% more efficient than previous approaches.

==> Figures/overview.tex <==

\includegraphics[width=1.0\linewidth]{Overview/overview_new}

\mycaption{Proposed \acs{medusa} Architecture} {
We focus on building independent task heads. 
This allows us to efficiently scale to a larger number of tasks thanks to the dual attention mechanisms. 
\textbf{(a)} Shared Feature Attention, selecting relevant backbone features for each task and scale through per-channel spatial attention. 
\textbf{(b)} Novel \acl{msa} head, combining task features at different scales to generate the final predictions.
}


==> Figures/qualitative.tex <==

\captionsetup{position=top}

\newcommand{\figsize}{0.19\linewidth}

\hfill
\subfloat[Input]{\includegraphics[width=\figsize]{Viz/gt/000132_image}}
\subfloat[GT]{\includegraphics[width=\figsize]{Viz/gt/000132_semseg}}
\subfloat[MT]{\includegraphics[width=\figsize]{Viz/mtl/000132_semseg}}
\subfloat[MTI-Net]{\includegraphics[width=\figsize]{Viz/mti_net/000132_semseg}}
\subfloat[\textbf{\acs{medusa}}]{\includegraphics[width=\figsize]{Viz/medusa/000132_semseg}}

\hfill
\subfloat{\includegraphics[width=\figsize]{Viz/gt/000132_depth}}
\subfloat{\includegraphics[width=\figsize]{Viz/mtl/000132_depth}}
\subfloat{\includegraphics[width=\figsize]{Viz/mti_net/000132_depth}}
\subfloat{\includegraphics[width=\figsize]{Viz/medusa/000132_depth}}

\hfill
\subfloat{\includegraphics[width=\figsize]{Viz/gt/000175_image}}
\subfloat{\includegraphics[width=\figsize]{Viz/gt/000175_semseg}}
\subfloat{\includegraphics[width=\figsize]{Viz/mtl/000175_semseg}} 
\subfloat{\includegraphics[width=\figsize]{Viz/mti_net/000175_semseg}}
\subfloat{\includegraphics[width=\figsize]{Viz/medusa/000175_semseg}}

\hfill
\subfloat{\includegraphics[width=\figsize]{Viz/gt/000175_depth}}
\subfloat{\includegraphics[width=\figsize]{Viz/mtl/000175_depth}} 
\subfloat{\includegraphics[width=\figsize]{Viz/mti_net/000175_depth}} 
\subfloat{\includegraphics[width=\figsize]{Viz/medusa/000175_depth}}

\mycaption{Qualitative Evaluation} { 
Through the proposed \ac{msa} heads, \acs{medusa}'s predictions are both globally consistent and have well defined borders. 
Results are on par with the current \ac{sota} while using less resources. 
}

==> Figures/resources.tex <==

\subfloat[]{\includegraphics[width=0.75\linewidth]{resources3} \label{fig:resources_a}}

\subfloat[]{\includegraphics[width=0.75\linewidth]{resources} \label{fig:resources_b}}

\mycaption{Resource Usage} {
Modelling the relationships between each pair of tasks and scales~\cite{Vandenhende2020d} results in a quadratic increase in paramters/GFLOPS \wrt the number of tasks. 
This does not scale well to an increasing number of tasks. 
\acs{medusa}'s independent task heads lead to a much more efficient scaling, while focusing on features that are more generic and reusable.
}

==> Medusa/Figures/intro.tex <==

\subfloat[Traditional]{\includegraphics[width=1\linewidth]{Intro/intro1_2}}

\subfloat[Proposed]{\includegraphics[width=1\linewidth]{Intro/intro2_2}}

\mycaption{Transferable Feature Learning}{
Current high-performing approaches to \acs{mtl} rely on connections between every combination of tasks, leading to a quadratic parameter complexity \wrt the number of tasks.
We maintain independent task heads, making it possible to easily add/remove new tasks \emph{a posteriori}.
The dual spatial attention mechanisms (\acs{sfa} \& \acs{msa}) allow us to maintain performance while scaling linearly and learning highly reusable feature representations.
See \fig{overview} for a full overview. 
}

==> Medusa/Figures/overview.tex <==

\includegraphics[width=1.0\linewidth]{Overview/overview_new}

\mycaption{Proposed \acs{medusa} Architecture} {
We focus on building independent task heads. 
This allows us to efficiently scale to a larger number of tasks thanks to the dual attention mechanisms. 
\textbf{(a)} Shared Feature Attention, selecting relevant backbone features for each task and scale through per-channel spatial attention. 
\textbf{(b)} Novel \acl{msa} head, combining task features at different scales to generate the final predictions.
}


==> Medusa/Figures/qualitative.tex <==

\captionsetup{position=top}

\newcommand{\figsize}{0.19\linewidth}

\hfill
\subfloat[Input]{\includegraphics[width=\figsize]{Viz/gt/000132_image}}
\subfloat[GT]{\includegraphics[width=\figsize]{Viz/gt/000132_semseg}}
\subfloat[MT]{\includegraphics[width=\figsize]{Viz/mtl/000132_semseg}}
\subfloat[MTI-Net]{\includegraphics[width=\figsize]{Viz/mti_net/000132_semseg}}
\subfloat[\textbf{\acs{medusa}}]{\includegraphics[width=\figsize]{Viz/medusa/000132_semseg}}

\hfill
\subfloat{\includegraphics[width=\figsize]{Viz/gt/000132_depth}}
\subfloat{\includegraphics[width=\figsize]{Viz/mtl/000132_depth}}
\subfloat{\includegraphics[width=\figsize]{Viz/mti_net/000132_depth}}
\subfloat{\includegraphics[width=\figsize]{Viz/medusa/000132_depth}}

\hfill
\subfloat{\includegraphics[width=\figsize]{Viz/gt/000175_image}}
\subfloat{\includegraphics[width=\figsize]{Viz/gt/000175_semseg}}
\subfloat{\includegraphics[width=\figsize]{Viz/mtl/000175_semseg}} 
\subfloat{\includegraphics[width=\figsize]{Viz/mti_net/000175_semseg}}
\subfloat{\includegraphics[width=\figsize]{Viz/medusa/000175_semseg}}

\hfill
\subfloat{\includegraphics[width=\figsize]{Viz/gt/000175_depth}}
\subfloat{\includegraphics[width=\figsize]{Viz/mtl/000175_depth}} 
\subfloat{\includegraphics[width=\figsize]{Viz/mti_net/000175_depth}} 
\subfloat{\includegraphics[width=\figsize]{Viz/medusa/000175_depth}}

\mycaption{Qualitative Evaluation} { 
Through the proposed \ac{msa} heads, \acs{medusa}'s predictions are both globally consistent and have well defined borders. 
Results are on par with the current \ac{sota} while using less resources. 
}

==> Medusa/Figures/resources.tex <==

\subfloat[]{\includegraphics[width=0.75\linewidth]{resources3} \label{fig:resources_a}}

\subfloat[]{\includegraphics[width=0.75\linewidth]{resources} \label{fig:resources_b}}

\mycaption{Resource Usage} {
Modelling the relationships between each pair of tasks and scales~\cite{Vandenhende2020d} results in a quadratic increase in paramters/GFLOPS \wrt the number of tasks. 
This does not scale well to an increasing number of tasks. 
\acs{medusa}'s independent task heads lead to a much more efficient scaling, while focusing on features that are more generic and reusable.
}

==> Medusa/Tables/ablation.tex <==

\mycaption{Spatial Attention Ablation Study} { 
The \acs{sfa} column indicates the presence of spatial attention between the shared backbone and the task heads.
Meanwhile, the \ac{msa} task head incorporates attention when combining each task's multi-scale features.
Both types of attention lead to clear improvements.
All models use the HRNet{\nbd}18 backbone. 
}

\begin{tabular}{@{}lllllll@{}}
\toprule
  & SFA & Head & N+E & Seg $\uparrow$ & Depth $\downarrow$ & $\acs{mtl-perf} \% \uparrow$ \\ 
\midrule
ST Baseline  && HRHead && 34.57 & 0.606 & +0.00 \\
MT Baseline  && HRHead && 33.21 & 0.614 & -2.63 \\
MT Baseline  && \textbf{\acs{msa}} && 35.58 & 0.598 & +2.12 \\
\hline
\textbf{\acs{medusa}} && HRHead & \cmark & 36.50 & 0.558 & +6.71 \\
\textbf{\acs{medusa}}  & \cmark & HRHead & \cmark & 36.64 & \nbest{0.553} & +7.31 \\ 
\textbf{\acs{medusa}} && \textbf{MSA} & \cmark & \nbest{37.14} & 0.555 & \nbest{+7.91} \\
\textbf{\acs{medusa}}  & \cmark & \textbf{\acs{msa}} & \cmark & \best{37.48} & \best{0.545} & \best{+9.24} \\ 
\bottomrule
\end{tabular}


==> Medusa/Tables/multi_task.tex <==

\mycaption{Multi-task Evaluation} {
When performing \ac{mtl} on NYUD-v2 \acs{medusa} is on par with the current \acs{sota}~\cite{Vandenhende2020d}, whilst using less resources (see \fig{resources}). 
This is due to the novel lightweight \ac{msa} task head.
We highlight the \best{best} and \nbest{next best} performing techniques.
}

\begin{tabular}{@{}lllllll@{}}
\toprule
 & Backbone & Head & N+E & Seg $\uparrow$ & Depth $\downarrow$ & $\acs{mtl-perf} \% \uparrow$ \\ 
\midrule
ST Baseline & ResNet-18 & DeepLab-v3+ && 35.77 & 0.600 & +0.00 \\
MT Baseline & ResNet-18 & DeepLab-v3+ && 35.74 & 0.597 & +0.12 \\
Cross-stitch \cite{Misra2016} & ResNet-18 & DeepLab-v3+ && 36.01 & 0.600 & +0.30 \\
NDDR-CNN \cite{Gao2019} & ResNet-18 & DeepLab-v3+ && 34.72 & 0.611 & -2.47 \\
MTAN \cite{Liu2019} & ResNet-18 & DeepLab-v3+ && 36.00 & 0.594 & +0.79 \\
\hline 
ST Baseline & HRNet-18 & HRHead && 34.57 & 0.606 & +0.00 \\
MT Baseline & HRNet-18 & HRHead && 33.21 & 0.614 & -2.63 \\
MTAN \cite{Liu2019} & HRNet-18 & DeepLab-v3+ && 35.25 & 0.581 & +3.02 \\
MTAN & HRNet-18 & DeepLab-v3+ & \cmark & 36.19 & 0.567 & +5.57 \\
PAD-Net \cite{Xu2018} & HRNet-18 & HRHead && 34.39 & 0.617 & -1.23 \\
PAD-Net & HRNet-18 & HRHead & \cmark & 35.46 & 0.604 & +1.43 \\ 
MTI-Net \cite{Vandenhende2020d} & HRNet-18 & HRHead && 36.94 & 0.559 & +7.26 \\
MTI-Net & HRNet-18 & HRHead & \cmark & \nbest{37.40} & \best{0.540} & \best{+9.48} \\
\hline
\textbf{\acs{medusa} (ours)} & HRNet-18 & \textbf{\acs{msa} (ours)} && 36.99 & 0.573 & +6.19 \\ 
\textbf{\acs{medusa}} & HRNet-18 & \textbf{\acs{msa}} & \cmark & \best{37.48} & \nbest{0.545} & \nbest{+9.24} \\ 
\bottomrule
\end{tabular}




==> Medusa/Tables/ufl.tex <==

\mycaption{Universal Feature Learning} {
We use the pretrained backbone features from \tbl{multi_task} to train task heads on new tasks on new datasets. 
The features learned by \acs{medusa} provide large improvements over the commonly used ImageNet pretrained features, despite the fact that we train with orders of magnitude less data. 
}

\begin{tabular}{@{}lllllll@{}}
\toprule
 & \multicolumn{3}{c}{NYUD-v2} & \multicolumn{3}{c}{PASCAL-Context} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
 &  Seg $\uparrow$ & Depth $\downarrow$ & $\acs{mtl-perf} \% \uparrow$ & Parts $\uparrow$ & Sal $\uparrow$ & $\acs{mtl-perf} \% \uparrow$ \\ 
\midrule
ST Baseline & 34.57 & 0.606 & +0.00 & 48.73 & 56.44 & +0.00 \\
MT Baseline & 33.21 & 0.614 & -2.63 & 36.13 & 51.96 & -12.93 \\
MTAN~\cite{Liu2019} & 36.19 & 0.567 & +5.57 & 47.37 & 57.84 & +4.26 \\
MTI-Net~\cite{Vandenhende2020d}  & \nbest{37.40} & \best{0.540} & \best{+9.48} & \nbest{51.50} & \nbest{60.19} & \nbest{+10.76} \\
\hline
\textbf{\acs{medusa}} & \best{37.48} & \nbest{0.545} & \nbest{+9.24} & \best{52.24} & \best{61.91} & \best{+13.18} \\
\bottomrule
\end{tabular}


==> Medusa/preamble.tex <==

\usepackage{xspace}
\usepackage{stmaryrd}  % Iverson brackets
%\usepackage{booktabs}  % Tables
\usepackage{pifont}    % Ding
%\usepackage{amssymb}
\usepackage[usenames,dvipsnames]{xcolor}
\usepackage{suffix}
%------------------------------------------------------------------------
%\usepackage{todonotes}
%\presetkeys{todonotes}{inline}{}  % Inline by default

%\usepackage{xcolor}
%\newcommand{\todo}[1]{\par \fcolorbox{black}{orange}{\parbox{0.9\linewidth}{#1}}}

%------------------------------------------------------------------------
\newcommand{\best}[1]{\textcolor{ForestGreen}{\textbf{#1}}}
\newcommand{\nbest}[1]{\textcolor{blue}{\underline{#1}}}

\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

\newcommand{\mycaption}[2]{\caption[#1]{\textbf{#1.}#2}}

%------------------------------------------------------------------------
\newcommand{\addfig}[3][!t]{
\begin{figure}[#1]
\centering
\input{#2}
\label{fig:#3}
\end{figure}
}

\WithSuffix\newcommand\addfig*[3][!t]{
\begin{figure*}[#1]
\centering
\input{#2}
\label{fig:#3}
\end{figure*}
}

\newcommand{\addtbl}[3][!t]{
\begin{table}[#1]
\renewcommand{\arraystretch}{1.2}
\centering
\input{#2}
\label{tbl:#3}
\end{table}
}

\WithSuffix\newcommand\addtbl*[3][!t]{
\begin{table*}[#1]
\renewcommand{\arraystretch}{1.2}
\centering
\input{#2}
\label{tbl:#3}
\end{table*}
}

%------------------------------------------------------------------------
% Useful symbols
\newcommand{\cmark}{\ding{51}}
\newcommand{\xmark}{\ding{55}}
\newcommand{\nbd}{\nobreakdash-} % Usage: "multi{\nbd}scale"

\newcommand{\ndim}[1]{#1{\nbd}D}
\newcommand{\pnorm}[1]{L\ensuremath{_#1}}

\newcommand{\codelink}{}

\newcommand{\heading}[1]{\noindent \textbf{#1.}}

%------------------------------------------------------------------------
% Inserting references
\newcommand{\fig}[1]{Figure~\ref{fig:#1}}
\newcommand{\tbl}[1]{Table~\ref{tbl:#1}}
\newcommand{\sct}[1]{Section~\ref{sec:#1}}
\newcommand{\eq}[1]{(\ref{eq:#1})}
\newcommand{\ch}[1]{Chapter~\ref{ch:#1}}

%------------------------------------------------------------------------
\newcommand{\myac}[1]{\text{\acs{#1}}}  % For inserting acronyms in acronyms

% Math operator utils
\DeclareMathOperator*{\mymax}{max}
\DeclareMathOperator*{\myargmax}{arg\,max}
\DeclareMathOperator*{\mymin}{min}
\DeclareMathOperator*{\myargmin}{arg\,min}
\DeclareMathOperator{\atantwo}{atan2}

\newcommand{\valmin}[2]{\mymin_{#1}\hspace{1mm}#2}
\newcommand{\argmin}[2]{\myargmin_{#1}\hspace{1mm}#2}
\newcommand{\valmax}[2]{\mymax_{#1}\hspace{1mm}#2}
\newcommand{\argmax}[2]{\myargmax_{#1}\hspace{1mm}#2}

% Avoid inline math linebreaks in awkward places
\binoppenalty=9999
\relpenalty=9999

%------------------------------------------------------------------------
\DeclareRobustCommand{\mysmallmath}[1]{\scriptscriptstyle{#1}}
\newcommand{\mysmallscript}[1]{\textnormal{\scriptsize \textsc{#1}}}

% Smaller minus symbol
\newcommand{\minus}{\scalebox{0.5}[0.75]{\ensuremath{-}}}
\newcommand{\inv}{\minus 1}

% Data types
\newcommand{\sca}[1]{\ensuremath{#1}}  						   % Non-bold
\newcommand{\vct}[1]{\ensuremath{\textbf{\MakeLowercase{#1}}}} % Lowercase/Bold
\newcommand{\mat}[1]{\ensuremath{\textbf{\MakeUppercase{#1}}}} % Uppercase/Bold
\newcommand{\set}[1]{\ensuremath{\MakeUppercase{#1}}} 	

\newcommand{\loss}{\ell}
\newcommand{\Loss}{\mathcal{L}}

\newcommand{\setreal}{\ensuremath{\mathbb{R}}}
\newcommand{\setnat}{\ensuremath{\mathbb{N}}}

%------------------------------------------------------------------------
% Brackets
\newcommand{\brackets}[3]{\ensuremath{\left#1 #2 \right#3}}
\newcommand{\mypar}[1]{\brackets{(}{#1}{)}}
\newcommand{\mybra}[1]{\brackets{\{}{#1}{\}}}
\newcommand{\mymag}[1]{\brackets{\|}{#1}{\|}} % These two 
\newcommand{\mynrm}[1]{\brackets{|}{#1}{|}}   % are flipped
\newcommand{\mysqb}[1]{\brackets{[}{#1}{]}}
\newcommand{\mybil}[1]{\brackets{\langle}{#1}{\rangle}}  % < a >
\newcommand{\myivr}[1]{\ensuremath{\llbracket #1 \rrbracket}}  % [[ a ]]

% Functions
\newcommand{\easyfunc}[2]{\ensuremath{#1\mypar{#2}}}                 % a(b)
\newcommand{\func}[3]{\ensuremath{ #1 = \easyfunc{#2}{#3} }}         % a = b(c)
\newcommand{\deffunc}[3]{\ensuremath{ \easyfunc{#1}{#2} = #3 }}      % a(b) = c

\newcommand{\easycond}[3]{\ensuremath{#1\mypar{#2 \middle| #3}}}     % a(b | c)
\newcommand{\cond}[4]{\ensuremath{ #1 = \easycond{#2}{#3}{#4} }}     % a = b(c | d)
\newcommand{\defcond}[4]{\ensuremath{ \easycond{#1}{#2}{#3} = #4 }}  % a(b | c) = d


% Sections
%------------------------------------------------------------------------

% Subsection
%........................................................................

% Equation/fig/table wrap
% =========================



==> Tables/ablation.tex <==

\mycaption{Spatial Attention Ablation Study} { 
The \acs{sfa} column indicates the presence of spatial attention between the shared backbone and the task heads.
Meanwhile, the \ac{msa} task head incorporates attention when combining each task's multi-scale features.
Both types of attention lead to clear improvements.
All models use the HRNet{\nbd}18 backbone. 
}

\begin{tabular}{@{}lllllll@{}}
\toprule
  & SFA & Head & N+E & Seg $\uparrow$ & Depth $\downarrow$ & $\acs{mtl-perf} \% \uparrow$ \\ 
\midrule
ST Baseline  && HRHead && 34.57 & 0.606 & +0.00 \\
MT Baseline  && HRHead && 33.21 & 0.614 & -2.63 \\
MT Baseline  && \textbf{\acs{msa}} && 35.58 & 0.598 & +2.12 \\
\hline
\textbf{\acs{medusa}} && HRHead & \cmark & 36.50 & 0.558 & +6.71 \\
\textbf{\acs{medusa}}  & \cmark & HRHead & \cmark & 36.64 & \nbest{0.553} & +7.31 \\ 
\textbf{\acs{medusa}} && \textbf{MSA} & \cmark & \nbest{37.14} & 0.555 & \nbest{+7.91} \\
\textbf{\acs{medusa}}  & \cmark & \textbf{\acs{msa}} & \cmark & \best{37.48} & \best{0.545} & \best{+9.24} \\ 
\bottomrule
\end{tabular}


==> Tables/multi_task.tex <==

\mycaption{Multi-task Evaluation} {
When performing \ac{mtl} on NYUD-v2 \acs{medusa} is on par with the current \acs{sota}~\cite{Vandenhende2020d}, whilst using less resources (see \fig{resources}). 
This is due to the novel lightweight \ac{msa} task head.
We highlight the \best{best} and \nbest{next best} performing techniques.
}

\begin{tabular}{@{}lllllll@{}}
\toprule
 & Backbone & Head & N+E & Seg $\uparrow$ & Depth $\downarrow$ & $\acs{mtl-perf} \% \uparrow$ \\ 
\midrule
ST Baseline & ResNet-18 & DeepLab-v3+ && 35.77 & 0.600 & +0.00 \\
MT Baseline & ResNet-18 & DeepLab-v3+ && 35.74 & 0.597 & +0.12 \\
Cross-stitch \cite{Misra2016} & ResNet-18 & DeepLab-v3+ && 36.01 & 0.600 & +0.30 \\
NDDR-CNN \cite{Gao2019} & ResNet-18 & DeepLab-v3+ && 34.72 & 0.611 & -2.47 \\
MTAN \cite{Liu2019} & ResNet-18 & DeepLab-v3+ && 36.00 & 0.594 & +0.79 \\
\hline 
ST Baseline & HRNet-18 & HRHead && 34.57 & 0.606 & +0.00 \\
MT Baseline & HRNet-18 & HRHead && 33.21 & 0.614 & -2.63 \\
MTAN \cite{Liu2019} & HRNet-18 & DeepLab-v3+ && 35.25 & 0.581 & +3.02 \\
MTAN & HRNet-18 & DeepLab-v3+ & \cmark & 36.19 & 0.567 & +5.57 \\
PAD-Net \cite{Xu2018} & HRNet-18 & HRHead && 34.39 & 0.617 & -1.23 \\
PAD-Net & HRNet-18 & HRHead & \cmark & 35.46 & 0.604 & +1.43 \\ 
MTI-Net \cite{Vandenhende2020d} & HRNet-18 & HRHead && 36.94 & 0.559 & +7.26 \\
MTI-Net & HRNet-18 & HRHead & \cmark & \nbest{37.40} & \best{0.540} & \best{+9.48} \\
\hline
\textbf{\acs{medusa} (ours)} & HRNet-18 & \textbf{\acs{msa} (ours)} && 36.99 & 0.573 & +6.19 \\ 
\textbf{\acs{medusa}} & HRNet-18 & \textbf{\acs{msa}} & \cmark & \best{37.48} & \nbest{0.545} & \nbest{+9.24} \\ 
\bottomrule
\end{tabular}




==> Tables/ufl.tex <==

\mycaption{Universal Feature Learning} {
We use the pretrained backbone features from \tbl{multi_task} to train task heads on new tasks on new datasets. 
The features learned by \acs{medusa} provide large improvements over the commonly used ImageNet pretrained features, despite the fact that we train with orders of magnitude less data. 
}

\begin{tabular}{@{}lllllll@{}}
\toprule
 & \multicolumn{3}{c}{NYUD-v2} & \multicolumn{3}{c}{PASCAL-Context} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
 &  Seg $\uparrow$ & Depth $\downarrow$ & $\acs{mtl-perf} \% \uparrow$ & Parts $\uparrow$ & Sal $\uparrow$ & $\acs{mtl-perf} \% \uparrow$ \\ 
\midrule
ST Baseline & 34.57 & 0.606 & +0.00 & 48.73 & 56.44 & +0.00 \\
MT Baseline & 33.21 & 0.614 & -2.63 & 36.13 & 51.96 & -12.93 \\
MTAN~\cite{Liu2019} & 36.19 & 0.567 & +5.57 & 47.37 & 57.84 & +4.26 \\
MTI-Net~\cite{Vandenhende2020d}  & \nbest{37.40} & \best{0.540} & \best{+9.48} & \nbest{51.50} & \nbest{60.19} & \nbest{+10.76} \\
\hline
\textbf{\acs{medusa}} & \best{37.48} & \nbest{0.545} & \nbest{+9.24} & \best{52.24} & \best{61.91} & \best{+13.18} \\
\bottomrule
\end{tabular}

